Few-shot Prompting for Pairwise Ranking: An Effective Non-Parametric Retrieval Model

A supervised ranking model, despite its advantage of being effective, usually involves complex processing - typically multiple stages of task-specific pre-training and fine-tuning. This has motivated researchers to explore simpler pipelines leveraging large language models (LLMs) that are capable of working in a zero-shot manner. However, since zero-shot inference does not make use of a training set of pairs of queries and their relevant documents, its performance is mostly worse than that of supervised models, which are trained on such example pairs. Motivated by the existing findings that training examples generally improve zero-shot performance, in our work, we explore if this also applies to ranking models. More specifically, given a query and a pair of documents, the preference prediction task is improved by augmenting examples of preferences for similar queries from a training set. Our proposed pairwise few-shot ranker demonstrates consistent improvements over the zero-shot baseline on both in-domain (TREC DL) and out-domain (BEIR subset) retrieval benchmarks. Our method also achieves a close performance to that of a supervised model without requiring any complex training pipeline.

==> src/intro.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.4\textwidth]{figs/workflow.pdf}
        \caption{Our proposed pairwise method for reranking a set of top-retrieved candidate documents via LLM-based inference. Different from \citet{qin2023large}, we provide additional context for LLM inference by including few-shot examples, each consisting of documents relevant to queries similar to the current input query as retrieved from a training set.        
        }
        \label{fig:prp}
    \end{figure}

Development of novel neural architectures and training methodologies \citep{pradeep2021expando,izacard2022unsupervised,10.1145/3404835.3463098,wang-etal-2023-simlm,karpukhin-etal-2020-dense} have substantially outperformed the unsupervised approaches.
Commonly, these neural approaches involve deep interactions between embedded representations of queries and documents \citep{dai2019contextaware,10.1145/3397271.3401075} thus overcoming the vocabulary mismatch problem of discrete term representations.
However, to achieve good performance, not only do these deep neural models require a large number of training data in the form of pairs of example queries and their relevant documents \citep{
10.1145/3477495.3531860,
saeed-etal-2021-neural},
but the effectiveness of these models also depends on a number of ad-hoc decision choices, e.g., the following.
\uls
\item \textit{Neural Architecture}, e.g., bi-encoder~\citep{dpr}, cross-encoder~\citep{monobert} or learned sparse models~\citep{epic};
\item \textit{Pre-Training Tasks} - to effectively capture retrieval specific term semantics \citep{gao-callan-2021-condenser,gao-etal-2021-coil};
\item \textit{Index construction} and the \textit{number of ranking stages}, e.g., sparse retrieval followed by reranking \citep{pradeep2021expando,DBLP:conf/ecir/LassanceDCT24}, vs. approximate inner product search on a dense vector index \citep{lin2020distilling,izacard2022unsupervised}, 
\item \textit{Negative Selection} - methodology for noise contrastive learning objective \citep{xiong2020approximate,10.1145/3404835.3462891,DBLP:conf/ecir/CohenIFK24};
\item \textit{Training Data Augmentation} via generative models
\citep{inpars, promptagator};
\item \textit{Distillation Strategies} - for effectively transferring the representational capabilities of larger models into smaller ones \citep{10.1145/3477495.3531799,lin2020distilling};
\item \textit{Curriculum Selection} - i.e., the order in which training samples are presented, for knowledge distillation \citep{he2023capstone, currdistill}.
\ule

With such a large number of decision choices available, it is difficult to converge on a set of `best practices' for designing the pipeline of a supervised ranker. Instead, in this paper, we present a relatively simple approach of leveraging the information from a training set of examples of query and relevant document pairs \textit{without requiring any parametric training}.
The motivation for this simple yet effective pipeline stems from the recent developments in large language models (LLMs), which exhibit emergent capabilities of modeling semantics \citep{ma2023zero}. By including a task definition and, optionally, examples of labelled or unlabelled data, these models can perform competitively on unseen tasks without fine-tuning \citep{sun2023chatgpt,qin2023large}. As such, they offer a compelling alternative to the highly data-driven fine-tuning currently applied in the field of neural retrieval.

Although recent work has employed LLMs for ranking, these approaches either simply use a zero-shot approach, thus not leveraging the benefits of a non-parametric memory (i.e., of a training set) \citep{qin2023large}, or they employ zero-shot inference only as an initial step for training data augmentation prior to train a supervised ranking model \cite{zhuang2022rankt5,ouyang2022training}. In contrast, our work, while on the one hand, employs an unsupervised approach (i.e., with no parametric training involved), it is able to make use of the training data of query-relevance examples via few-shot prompting on the other.

More specifically, as outlined in Figure \ref{fig:prp}, in our approach, following the methodology of \citep{qin2023large} we input a query and a pair of documents seeking to estimate the relative preferential order between the pair. However, in contrast to the PRP (pairwise rank prompting) method of \citet{qin2023large}, we input a set of queries (from an available training set) that are related to the current query in terms of an abstract similarity measure. This is motivated from the well-known cognitive bias \textit{attribute substitution} effect in psychology, where to answer an unknown question, human brains \textit{recollect known answers to related questions} and eventually \textit{process information from them to answer the unknown one} \citep{Kahneman2002a,https://doi.org/10.1111/cogs.12395}.

In our work, we emulate this behavior of attribute substitution heuristics on LLMs, where in additional context \citep{brown2020advances}, we provide examples of related queries and their relevant documents. The hypothesis is that LLMs, with their inherent language processing abilities, should be able to make a more informed judgment of pairwise relevance by processing the examples provided.

This proposed workflow requires investigating a number of research questions and challenges including: ``how to retrieve an effective set of related queries for a given input?'', and ``what is the downstream effect of the similarity of the information needs of the related queries''. Our experiments show that an embedding-based neighborhood to retrieve related queries yields better downstream effectiveness than a lexical model, and we also show that a small number of examples can, in fact, lead to consistent improvements over the zero-shot PRP approach \citep{qin2023large}.
Our experiments also demonstrate the potential of this unsupervised method for out-of-domain generalization. More specifically, we show that examples queries from MS-MARCO lead to improvements on TREC Covid and SciFact test collections.
The source code of our proposed LLM-based few-shot ranker\footnote{\url{https://github.com/nilanjansb/fewshot_prp}} is made available for research purposes.







==> src/limitations.tex <==
\section*{Ethical Statement}
Noting to declare.

\section*{Limitations}
We mainly focus on the open-source lightweight LLMs ($\leq$7B) and whether the few-shot performance gains are much higher with larger LLMs (such as LLaMa-70B, GPT-3.5 or GPT-4) is yet to be investigated.
We also consider only the `All-Pairs' method for reranking the top-100 documents, which was one of the techniques used in \cite{qin2023large}. While \cite{qin2023large} proposed a pseudo-sorting algorithm as an approximate strategy requiring with linear complexity (as opposed to quadratic complexity for an exhaustive pairwise setting) and \citep{setwiserank} proposed further improvements using more effective sorting algorithms, our approach can be trivially applied under these setting to improve efficiency.




==> src/rel_new.tex <==





\para{Zero-shot Information Retrieval with LLMs}
\looseness -1 Generative language models exhibit generalization capabilities beyond the tasks on which they are trained~\citep{instructgpt,touvron2023llama}. Naturally, this has led to a number of effective zero-shot approaches to NLP tasks.
\looseness -1 \citet{sun2023chatgpt} first proposed the use of LLMs as cross-encoders in a list-wise ranking setting.
Similar results were observed by \citet{lrl} using a different prompting strategy.
A common thread of work proposes distilling list-wise closed source models into smaller decoder-only architectures~\citep{pradeep2023rankvicuna, pradeep2023rankzephyr, rankwogpt}. They report that, in some cases, a student model could outperform a significantly larger teacher model~\citep{pradeep2023rankzephyr}. Beyond list-wise ranking, LLMs have additionally been applied in a bi-encoder setting \citep{ma2023fine}. 

\citet{qin2023large} first applied large language models to pair-wise ranking, finding that in a truly zero-shot setting, such an approach was competitive on out-of-domain benchmarks.
\citet{setwiserank} further improved both the efficiency and effectiveness of pair-wise ranking.


\para{In-Context Learning (ICL)}
In-context learning or few-shot learning is an inference strategy that differs from the standard notion of supervised learning in the sense that labeled examples are appended to a model instruction improving effectiveness in an out-of-domain downstream task \citep{ni2021large, li-etal-2022-encoder}.
Though initially considered to guide sequence generation in tasks such as question answering and abstractive summarization \citep{li-etal-2023-shot,tang-etal-2023-context}, ICL has been shown to be effective in classification-style tasks \citep{lu-etal-2022-fantastically,milios-etal-2023-context} and, therefore, could be effective in a cross-encoder setting for ranking. In terms of example selection for ICL, prior work has found that conditioning chosen examples on the current test instance is effective~\citep{nie2022improving, selfimprove}.





==> src/result_apdx.tex <==
\begin{table*}[t]
\centering
\caption{
A comparison to show the effect of changing the phase-one retriever to Contriver with two different neighborhood similarity functions. Each one-shot result reported in this table is an average over 5 runs with the standard
deviations included in superscript. The best scores across all unsupervised approaches are bold-faced, and the overall best
result in a group is underlined. Letters a to d are used to indicate the statistical significance of a retriever with Zephyr-0S,Zephyr-LEX-1S, Zephyr-SEM-1S, and monoT5.
\label{tab:allpair_scores_apdx}
}
\small
\begin{adjustbox}{width=.95\textwidth}
\begin{tabular}{@{}ll llllll@{}}
\toprule
& & \multicolumn{3}{c}{TREC DL'19} & \multicolumn{3}{c}{TREC DL'20}\\
\cmidrule(r){3-5} \cmidrule(r){6-8}
Type & Retriever & $\mnjs$ & AP@100 & nDCG@10 & $\mnjs$ & AP@100 & nDCG@10 \\
\midrule
\multirow{2}{*}{Baseline}  & Contriever & n/a & .3400 & .5888 & n/a & .3694 & .5845 \\
\cmidrule(r){2-8}
& Zephyr-0S & n/a & .3693 & .6391 & n/a & .3637 & .5758 \\
\midrule
\multirow{6}{*}{Ours} & \multicolumn{7}{c}{ BM25 >> Few-shot PRP}  \\
\cmidrule(r){2-8}
& Zephyr-LEX-1S & .267 & $\resdev{.3447}{.0019}$$^a$ & $\resdev{.6742}{.0005}$$^a$ & .244 & $\resdev{.3793}{.0052}$$^{a bc} $ & $\resdev{.6457}{.0077}$$^{a bc}$\\
& Zephyr-SEM-1S & .352 & $\resdev{\underline{.3512}}{.0041}$$^a$ & $\resdev{\underline{.6785}}{.0028}$$^a$ & .370 & $\resdev{\underline{.3824}}{.0019}$$^{a bc}$ & $\resdev{\underline{.6480}}{.0033}$$^{a  bc} $\\
\cmidrule(r){2-8}
&  \multicolumn{7}{c}{Contriever >> Few-shot PRP}  \\
\cmidrule(r){2-8}
& Zephyr-LEX-1S & .267 & $\resdev{\textbf{.4145}}{.0013}$$^{abcd}$ & $\resdev{\textbf{.6889}}{.0021}$$^a$ & .244 & $\resdev{.4219}{.0015}$$^{a bc} $ & $\resdev{.6677}{.0018}$$^{a bc}$\\
& Zephyr-SEM-1S & .352 & $\resdev{.3940}{.0012}$$^{ab}$ & $\resdev{.6679}{.0036}$$^a$ & .370 & $\resdev{\textbf{.4231}}{.0016}$$^{a bc}$ & $\resdev{\mathbf{.6680}}{.0010}$$^{a  bc} $\\
\cmidrule{1-8}
\rowcolor{lightgray}
Supervised & monoT5 & n/a & \textbf{.3570}$^{a}$ & \textbf{.6998}$^{a}$ & n/a & \textbf{.3970}$^{a}$ & \textbf{.6729}$^{a}$ \\

\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}


==> src/result_ood_apdx.tex <==
\begin{table}[t]
\centering
\caption{
Evaluating (nDCG@10) re-ranking performance on top-20 Contriever retrieved documents in out-of-domain settings. Letters $a$ to $d$ are used to indicate the statistical significance of a retriever with Zephyr-0S, Zephyr-LEX-1S, Zephyr-SEM-1S, and monoT5 (paired $t$-test with $p=0.05$).
\label{tab:beir_results_apdx}
}
\small
\begin{adjustbox}{width=.95\columnwidth}
\begin{tabular}{@{}l@{~~}c@{~~}c@{~~}c@{~~}c@{}}
\toprule
& \multicolumn{2}{c}{TREC Covid} & \multicolumn{2}{c}{SciFact} \\
\cmidrule(r){2-3}
\cmidrule(r){4-5}
Retriever& $\mnjs$ & nDCG@10 & $\mnjs$ & nDCG@10 \\
\midrule
BM25 & n/a & .5781 & n/a & .6722\\
Contriever & n/a & .3723 & n/a & .6081\\
\cmidrule(r){1-5}
\multicolumn{5}{c}{BM25 >> Few-shot PRP}\\
\cmidrule(r){1-5}
Zephyr-0S & n/a & .6571 & n/a & .6872 \\
Zephyr-LEX-1S & .130 & \textbf{.6790}$^{a d}$ & .093 & \textbf{.6988} \\
Zephyr-SEM-1S & .094 & .6753$^{d}$ & .067 & .6880 \\
\cmidrule(r){1-5}
\multicolumn{5}{c}{Contriever >> Few-shot PRP}\\
\cmidrule(r){1-5}
Zephyr-0S & n/a & .4989 & n/a & .5628 \\
Zephyr-LEX-1S & .130 & .4963 & .093 & .6264 \\
Zephyr-SEM-1S & .094 & .4922 & .067 & .6027 \\
\midrule
\rowcolor{lightgray}
monoT5 & n/a & .6376 & n/a & \textbf{.7204}$^{a c}$ \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}




==> src/results_ood.tex <==
\begin{table}[t]
\centering
\caption{
Evaluating (nDCG@10) re-ranking performance on top-20 BM25 retrieved documents in out-of-domain settings. The query-document relevance pairs are retrieved from MS MARCO to construct the ICL example sets for other test collections. Here, only the BM25 and Zephyr-0S baselines, supervised monoT5 ranker, and our localized 1S methods are compared. Letters $a$ to $d$ are used to indicate the statistical significance of a retriever with Zephyr-0S, Zephyr-LEX-1S, Zephyr-SEM-1S, and monoT5 (paired $t$-test with $p=0.05$).
\label{tab:beir_results}
}
\small
\begin{adjustbox}{width=.95\columnwidth}
\begin{tabular}{@{}l@{~~}c@{~~}c@{~~}c@{~~}c@{}}
\toprule
& \multicolumn{2}{c}{TREC Covid} & \multicolumn{2}{c}{SciFact} \\
\cmidrule(r){2-3}
\cmidrule(r){4-5}
Retriever& $\mnjs$ & nDCG@10 & $\mnjs$ & nDCG@10 \\
\midrule
BM25 & n/a & .5781 & n/a & .6722\\
Contriever & n/a & .4499 & n/a & .6477\\
Zephyr-0S & n/a & .6571 & n/a & .6872 \\
Zephyr-LEX-1S & .130 & \textbf{.6790}$^{a d}$ & .093 & \textbf{.6988} \\
Zephyr-SEM-1S & .094 & .6753$^{d}$ & .067 & .6880 \\
\midrule
\rowcolor{lightgray}
monoT5 & n/a & .6376 & n/a & \textbf{.7204}$^{a c}$ \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}





==> src/srp_table.tex <==
\begin{table*}[t]
\centering
\caption{
Analysis of our few-shot extension to Pointwise and Setwise ranking strategies.
\label{tab:srp_scores}
}
\small
\begin{adjustbox}{width=.85\textwidth}
\begin{tabular}{@{}ll llllll@{}}
\toprule
& & \multicolumn{3}{c}{TREC DL'19} & \multicolumn{3}{c}{TREC DL'20}\\
\cmidrule(r){3-5} \cmidrule(r){6-8}
Type & Retriever & $\mnjs$ & AP@100 & nDCG@10 & $\mnjs$ & AP@100 & nDCG@10 \\
\midrule
\multirow{3}{*}{Pointwise} & Zephyr-0S & n/a & $.2268$ & $.5195$ & n/a & $.2008$ & $.5690$ \\
& Zephyr-1S & .041 & $.2402$ & $.5271$ & .370 & $.1893$ & $.5503$ \\
& Zephyr-LEX-1S & .267 & $.2416$ & $.5559$ & .244 & $.1841$ & $.5610$\\

\cmidrule{2-8}
\multirow{4}{*}{Setwise} & Zephyr-0S & n/a & $.3122$ & $.6143$ & n/a & $.3468$ & $.5953$ \\
& Zephyr-1S & .041 & $.2292$ & $.6176$ & .029 & $.3517$ & $.6067$ \\
& Zephyr-LEX-1S & .267 & $.3080$ & $.6417$ & .244 & $.3613$ & $.6101$ \\
& Zephyr-SEM-1S & .352 & $.2993$ & $.6317$ & .370 & $.3373$ & $.5985$ \\

\bottomrule
\end{tabular}
\end{adjustbox}
\end{table*}

